Multi-Agent Motion Planning For Differential Drive Robots Through Stationary State Search

Multi-Agent Motion Planning (MAMP) finds various applications in fields such as traffic management, airport operations, and warehouse automation. In many of these environments, differential drive robots are commonly used. These robots have a kinodynamic model that allows only in-place rotation and movement along their current orientation, subject to speed and acceleration limits. However, existing Multi-Agent Path Finding (MAPF)-based methods often use simplified models for robot kinodynamics, which limits their practicality and realism. In this paper, we introduce a three-level framework called MASS to address these challenges. MASS combines MAPF-based methods with our proposed stationary state search planner to generate high-quality kinodynamically-feasible plans. We further extend MASS using an adaptive window mechanism to address the lifelong MAMP problem. Empirically, we tested our methods on the single-shot grid map domain and the lifelong warehouse domain. Our method shows up to 400% improvements in terms of throughput compared to existing methods.

==> docs/checklist.tex <==
\section{Reproducibility Checklist}
This paper:

\begin{itemize}
    \item \textbf{Yes} - Includes a conceptual outline and/or pseudocode description of AI methods introduced: (yes/partial/no/NA)
    \item \textbf{Yes} - Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: (yes/no)
    \item \textbf{Yes} - Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper: (yes/no)
    \item \textbf{Yes} - Does this paper make theoretical contributions? (yes/no)
    
    \textbf{If yes, please complete the list below.}
    \begin{itemize}
        % \item \textbf{Yes} - All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
        % \item \textbf{Yes} - All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
        % \item \textbf{Yes} - Proofs of all novel claims are included. (yes/partial/no)
        % \item \textbf{Yes} - Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
        % \item \textbf{Yes} - Appropriate citations to theoretical tools used are given. (yes/partial/no)
        % \item \textbf{Yes} - All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
        % \item \textbf{Yes} - All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
        \item \textbf{Yes} - All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
        \item \textbf{Yes} - All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
        \item \textbf{Yes} - Proofs of all novel claims are included. (yes/partial/no)
        \item \textbf{Yes} - Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
        \item \textbf{Yes} - Appropriate citations to theoretical tools used are given. (yes/partial/no)
        \item \textbf{Yes} - All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
        \item \textbf{Yes} - All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
    \end{itemize}

    \item \textbf{Yes} - Does this paper rely on one or more datasets? (yes/no)
    
    \textbf{If yes, please complete the list below.}
    \begin{itemize}
        \item \textbf{Yes} - A motivation is given for why the experiments are conducted on the selected datasets. (yes/partial/no/NA)
        \item \textbf{Yes} - All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
        \item \textbf{Yes} - All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
        \item \textbf{Yes} - All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
        \item \textbf{Yes} - All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
        \item \textbf{Yes} - All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
    \end{itemize}
    
    \item \textbf{Yes} - Does this paper include computational experiments? (yes/no)
    
    \textbf{If yes, please complete the list below.}
    \begin{itemize}
        \item \textbf{Yes} - Any code required for pre-processing data is included in the appendix. (yes/partial/no)
        \item \textbf{Yes} - All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
        \item \textbf{Yes} - All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
        \item \textbf{Yes} - All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. (yes/partial/no)
        \item \textbf{Yes} - If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
        \item \textbf{Yes} - This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
        \item \textbf{Yes} - This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)
        \item \textbf{Yes} - This paper states the number of algorithm runs used to compute each reported result. (yes/no)
        \item \textbf{Yes} - Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
        \item \textbf{Yes} - The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
        \item \textbf{Yes} - This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)
        \item \textbf{Yes} - This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)
    \end{itemize}
\end{itemize}
% \section{Reproducibility Checklist}

% \begin{enumerate}

% \item This paper:
% \begin{enumerate}
%     \item  Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) yes
%     \item Clearly delineates statements that are opinions, hypotheses, and speculations from objective facts and results (yes/no) yes
%    \item Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes/no) yes
% \end{enumerate}

% \item Does this paper make theoretical contributions? (yes/no)
%      If yes, please complete the list below. no
% \begin{enumerate}
%   \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
     
%   \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
     
%   \item Proofs of all novel claims are included. (yes/partial/no)
     
%   \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
     
%   \item Appropriate citations to theoretical tools used are given. (yes/partial/no)

%   \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)

%   \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
     
% \end{enumerate}

% \item Does this paper rely on one or more datasets? (yes/no)
% If yes, please complete the list below. yes
% \begin{enumerate}
%   \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) yes
     
%   \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) yes
     
%   \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) yes
     
%   \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) yes
     
%   \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) yes
  
%   \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) NA
     
% \end{enumerate}

% \item Does this paper include computational experiments? (yes/no)
% If yes, please complete the list below. yes

% \begin{enumerate}
%     \item Any code required for pre-processing data is included in the appendix. (yes/partial/no). yes
     
%     \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) yes

%     \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) yes

%     \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) yes
     
%     \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) yes
  
%     \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) yes
     
%     \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) yes

%     \item This paper states the number of algorithm runs used to compute each reported result. (yes/no) no
     
%     \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) yes
     
%     \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) yes


%     \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) yes

%     \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) NA
     
% \end{enumerate}

% \end{enumerate}
